On the Performance of Handover Mechanisms for Non-Terrestrial Networks

Next-generation wireless networks require massive connectivity and ubiquitous coverage, for which non-terrestrial networks (NTNs) are a promising enabler. However, NTNs, especially non-geostationary satellites bring about challenges such as increased handovers (HOs) due to the moving coverage area of the satellite on the ground. Accordingly, in this work, we compare the conventional measurement-based HO triggering mechanism with other alternatives such as distance, elevation angle, and timer-based methods in terms of the numbers of HOs, ping-pong HOs, and radio link failures. The system-level simulations, carried out in accordance with the 3GPP model, show that the measurement-based approach can outperform the other alternatives provided that appropriate values of hysteresis/offset margins and time-to-trigger parameters are used. Moreover, future directions regarding this work are also provided at the end.

==> AcronymList.tex <==
\usepackage{etoolbox}
\makeatletter
\newif\ifAC@uppercase@first%
\def\Aclp#1{\AC@uppercase@firsttrue\aclp{#1}\AC@uppercase@firstfalse}%
\def\AC@aclp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acl{#1}s%
	\fi%
}%
\def\Acp#1{\AC@uppercase@firsttrue\acp{#1}\AC@uppercase@firstfalse}%
\def\AC@acp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@ac{#1}s%
	\fi%
}%
\def\Acfp#1{\AC@uppercase@firsttrue\acfp{#1}\AC@uppercase@firstfalse}%
\def\AC@acfp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acf{#1}s%
	\fi%
}%
\def\Acsp#1{\AC@uppercase@firsttrue\acsp{#1}\AC@uppercase@firstfalse}%
\def\AC@acsp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acs{#1}s%
	\fi%
}%
\edef\AC@uppercase@write{\string\ifAC@uppercase@first\string\expandafter\string\MakeUppercase\string\fi\space}%
\def\AC@acrodef#1[#2]#3{%
	\@bsphack%
	\protected@write\@auxout{}{%
		\string\newacro{#1}[#2]{\AC@uppercase@write #3}%
	}\@esphack%
}%
\def\Acl#1{\AC@uppercase@firsttrue\acl{#1}\AC@uppercase@firstfalse}
\def\Acf#1{\AC@uppercase@firsttrue\acf{#1}\AC@uppercase@firstfalse}
\def\Ac#1{\AC@uppercase@firsttrue\ac{#1}\AC@uppercase@firstfalse}
\def\Acs#1{\AC@uppercase@firsttrue\acs{#1}\AC@uppercase@firstfalse}
\robustify\Aclp
\robustify\Acfp
\robustify\Acp
\robustify\Acsp
\robustify\Acl
\robustify\Acf
\robustify\Ac
\robustify\Acs
\makeatother

\acrodef{PDCP}[PDCP]{packet data convergence protocol}
\acrodef{RATs}[RATs]{radio access technologies}
% \acrodefplural{RAT}[RAT]{radio access technologies}
\acrodef{AP}[AP]{access point}
\acrodef{MP-TCP}[MP-TCP]{Multipath transmission control protocol}
\acrodef{5QI}[5QI]{\ac{5G} \ac{QoS} identifier}
\acrodef{NSI}[NSI]{network slice instance}
\acrodef{ATSSS}[ATSSS]{access traffic steering, switching and splitting}
\acrodef{CA}[CA]{coordination area}
\acrodef{TRP}[TRP]{transmission-reception point}
\acrodef{SON}[SON]{self-organizing network}
\acrodef{V2X}[V2X]{vehicle-to-everything}
\acrodef{eMBB}[eMBB]{enhanced mobile broadband}
\acrodef{mMTC}[mMTC]{massive machine type communication}
\acrodef{uRLLC}[uRLLC]{ultra-reliable low latency communication}
\acrodef{CoMP}[CoMP]{coordinated multipoint}
\acrodef{LTE}[LTE]{Long Term Evolution}
\acrodef{LTE-A}[LTE-A]{LTE-Advanced}
\acrodef{3GPP}[3GPP]{3rd Generation Partnership Project}
\acrodef{FFR}[FFR]{fractional frequency reuse}
\acrodef{SFR}[SFR]{soft frequency reuse}
\acrodef{ICI}[ICI]{inter-cell interference}
\acrodef{ICIC}[ICIC]{inter-cell interference coordination}
\acrodef{eICIC}[eICIC]{enhanced \ac{ICIC}}
\acrodef{ABS}[ABS]{absolute blank subframe}
\acrodef{TP}[TP]{transmission point}
\acrodef{CSI}[CSI]{channel state information}
\acrodef{eNB}[eNB]{eNodeB}
\acrodef{RAN}[RAN]{radio access network}
\acrodef{C-RAN}[C-RAN]{cloud-RAN}
\acrodef{RRH}[RRH]{remote radio head}
\acrodef{BBU}[BBU]{baseband unit}
\acrodef{CS}[CS]{coordinated scheduling}
\acrodef{CB}[CB]{coordinated beamforming}
\acrodef{JT}[JT]{joint transmission}
\acrodef{NC-JT}[NC-JT]{non-coherent \ac{JT}}
\acrodef{C-JT}[C-JT]{coherent \ac{JT}}
\acrodef{DPS}[DPS]{dynamic point selection}
\acrodef{TTI}[TTI]{transmission time interval}
\acrodef{UE}[UE]{user equipment}
\acrodef{RNTP}[RNTP]{relative narrowband transmission power}
\acrodef{eRNTP}[eRNTP]{enhanced \ac{RNTP}}
\acrodef{OI}[OI]{overload indicator}
\acrodef{HII}[HII]{high interference indicator}
\acrodef{HG}[HG]{Hermite-Gaussian}
\acrodef{CQI}[CQI]{channel quality indicator}
\acrodef{PMI}[PMI]{precoding matrix indicator}
\acrodef{RI}[RI]{rank indicator}
\acrodef{HetNet}[HetNet]{heterogeneous network}
\acrodef{mmWave}[mmWave]{millimeter wave}
\acrodef{SINR}[SINR]{signal-to-interference-plus-noise ratio}
\acrodef{SC}[SC]{single-carrier}
\acrodef{SM-OFDM}[SM-OFDM]{Spatial modulation-OFDM}
\acrodef{GB}[GB]{guard band}
\acrodef{DL}[DL]{downlink}
\acrodef{FFT}[FFT]{fast Fourier transform}
\acrodef{IFFT}[IFFT]{inverse fast Fourier transform}
\acrodef{CP}[CP]{cyclic prefix}
\acrodef{GBR}[GBR]{guaranteed bit-rate}
\acrodef{GFDM}[GFDM]{generalized orthogonal frequency division multiplexing}
\acrodef{RSRP}[RSRP]{reference signal received power}
\acrodef{RSRQ}[RSRQ]{reference signal received quality}
\acrodef{CSI-RSRP}[CSI-RSRP]{CSI-reference signal received power}
\acrodef{se}[SE]{spectral efficiency}
\acrodef{5G}[5G]{fifth generation}
\acrodef{6G}[6G]{sixth generation}
\acrodef{4G}[4G]{fourth generation}
\acrodef{papr}[PAPR]{peak-to-average power ratio}
\acrodef{isi}[ISI]{intersymbol interference}
\acrodef{wdm}[WDM]{waveform division multiplexing}
\acrodef{noma}[NOMA]{non-orthogonal multiple access}
\acrodef{MIMO}[MIMO]{multiple-input multiple-output}
\acrodef{GCoMP}[GCoMP]{generalized CoMP}
\acrodef{CU}[CU]{central unit}
\acrodef{DU}[DU]{distributed unit}
\acrodef{RU}[RU]{remote unit}
\acrodef{FH}[FH]{fronthaul}
\acrodef{LoS}[LoS]{line-of-sight}
\acrodef{NLoS}[NLoS]{non-line-of-sight}
\acrodef{TBS}[TBS]{terrestrial base station}
\acrodef{FBS}[FBS]{flying base station}
\acrodef{PLS}[PLS]{physical layer security}
\acrodef{PRB}[PRB]{physical resource block}
\acrodef{PSK}[PSK]{phase-shift keying}
\acrodef{QAM}[QAM]{quadrature amplitude modulation}
\acrodef{ostbc}[OSTBC]{orthogonal space time block codes}
\acrodef{OOBE}[OOBE]{out-of-band emission}
\acrodef{svd}[SVD]{singular value decomposition}
\acrodef{MAC}[MAC]{medium access control}
\acrodef{PHY}[PHY]{physical}
\acrodef{THz}[THz]{terahertz}
\acrodef{RIS}[RIS]{reconfigurable intelligent surface}
\acrodef{QoS}[QoS]{quality of service}
\acrodef{ITS}[ITS]{intelligent transportation system}
% \acrodef{TRxP}[TRxP]{transmission reception point}
\acrodef{HO}[HO]{handover}
\acrodef{PPHO}[PP HO]{ping-pong handover}
\acrodef{TUBITAK}[TUBITAK]{Scientific and Technological Research Council of Turkey}
\acrodef{MBB}[MBB]{\textit{Make-Before-Break}}
\acrodef{RACH}[RACH]{\textit{Random Access Channel}}
\acrodef{eMTC}[eMTC]{\textit{enhanced machine type communication}}
\acrodefplural{GBR}[GBR]{guaranteed bit rate}
\acrodef{RB}[RB]{resource block}
\acrodef{PPP}[PPP]{Poisson point process}
\acrodef{ZF}[ZF]{zero-forcing}
\acrodef{RSS}[RSS]{received signal strength}
\acrodef{RSSI}[RSSI]{received signal strength indicator}
\acrodef{CIR}[CIR]{channel impulse response}
\acrodef{CP}[CP]{cyclic prefix}
\acrodef{ISI}[ISI]{inter-symbol interference}
\acrodef{UAV}[UAV]{unmanned aerial vehicle}
\acrodef{ISD}[ISD]{inter-site distance}
\acrodef{OFDM}[OFDM]{orthogonal frequency-division multiplexing}
\acrodef{BER}[BER]{bit error rate}
\acrodef{CSF}[CSF]{channel shortening filter}
\acrodef{AWGN}[AWGN]{additive white Gaussian noise}
\acrodef{TDD}[TDD]{time division duplex}
\acrodef{SNR}[SNR]{signal-to-noise ratio}
\acrodef{MSSNR}[MSSNR]{maximum shortening signal-to-noise ratio}
\acrodef{PSD}[PSD]{power spectral density}
\acrodef{QPSK}[QPSK]{Quadrature Phase Shift Keying}
\acrodef{NTN}[NTN]{non-terrestrial network}
\acrodef{RLF}[RLF]{radio link failure}
\acrodef{LEO}[LEO]{low Earth orbit}
\acrodef{TTT}[TTT]{time-to-trigger}
\acrodef{FSPL}[FSPL]{free space path loss}
\acrodef{SF}[SF]{shadowing fading}
\acrodef{CL}[CL]{clutter loss}
\acrodef{CHO}[CHO]{conditional handover}
\acrodef{PP}[PP]{ping-pong}
\acrodef{RW}[RW]{random walk}
\acrodef{EIRP}[EIRP]{equivalent isotropically radiated power}
\acrodef{GPS}[GPS]{Global Positioning System}

